LanPose: Language-Instructed 6D Object Pose Estimation for Robotic Assembly

Comprehending natural language instructions is a critical skill for robots to cooperate effectively with humans. In this paper, we aim to learn 6D poses for roboticassembly by natural language instructions. For this purpose, Language-Instructed 6D Pose Regression Network (LanPose) is proposed to jointly predict the 6D poses of the observed object and the corresponding assembly position. Our proposed approach is based on the fusion of geometric and linguistic features, which allows us to finely integrate multi-modality input and map it to the 6D pose in SE(3) space by the cross-attention mechanism and the language-integrated 6D pose mapping module, respectively. To validate the effectiveness of our approach, an integrated robotic system is established to precisely and robustly perceive, grasp, manipulate and assemble blocks by language commands. 98.09 and 93.55 in ADD(-S)-0.1d are derived for the prediction of 6D object pose and 6D assembly pose, respectively. Both quantitative and qualitative results demonstrate the effectiveness of our proposed language-instructed 6D pose estimation methodology and its potential to enable robots to better understand and execute natural language instructions.

==> figs/2_system.tex <==
\begin{figure*}
	\centering
	\vspace{2mm}
	\includegraphics[width = 0.99\linewidth]{figs/pic_2_system.pdf}\vspace{-2mm}
	\caption{Flow chart of our system. Given an RGB image and a description text, we first locate the base object and the target object by a 2D visual grounding network. The object ROIs are then fed into our proposed \textit{Language-Instructed 6D Pose Regression Network} (LanPose) to jointly predict the object pose and the assembly position pose. Subsequently, the target block is grasped, manipulated and assembled precisely to the base block. }
	\label{fig:system}
\end{figure*}

==> figs/3_network.tex <==
\begin{figure*}
	\centering
	\vspace{2mm}
	\includegraphics[width = 0.85\linewidth]{figs/pic_3_network.pdf}\vspace{-4mm}
% 	\vspace{-0.2mm}
	\caption{Overview of LanPose. Given the ROI of the block, our network predicts several intermediate geometric feature maps and then directly regress the 6D base object pose. Simultaneously, the language instruction is fed to RoBRETa to produce the text encoding. Then the concatenation of the linguistic and geometric features is mapped to the 6D assembly position pose. }
% 	\vspace{-2mm}
	\label{fig:network}
\end{figure*}
